DiffScale: Continuous Downscaling and Bias Correction of Subseasonal Wind Speed Forecasts using Diffusion Models

Renewable resources are strongly dependent on local and large-scale weather situations. Skillful subseasonal to seasonal (S2S) forecasts -- beyond two weeks and up to two months -- can offer significant socioeconomic advantages to the energy sector. This study aims to enhance wind speed predictions using a diffusion model with classifier-free guidance to downscale S2S forecasts of surface wind speed. We propose DiffScale, a diffusion model that super-resolves spatial information for continuous downscaling factors and lead times. Leveraging weather priors as guidance for the generative process of diffusion models, we adopt the perspective of conditional probabilities on sampling super-resolved S2S forecasts. We aim to directly estimate the density associated with the target S2S forecasts at different spatial resolutions and lead times without auto-regression or sequence prediction, resulting in an efficient and flexible model. Synthetic experiments were designed to super-resolve wind speed S2S forecasts from the European Center for Medium-Range Weather Forecast (ECMWF) from a coarse resolution to a finer resolution of ERA5 reanalysis data, which serves as a high-resolution target. The innovative aspect of DiffScale lies in its flexibility to downscale arbitrary scaling factors, enabling it to generalize across various grid resolutions and lead times -without retraining the model- while correcting model errors, making it a versatile tool for improving S2S wind speed forecasts. We achieve a significant improvement in prediction quality, outperforming baselines up to week 3.

==> figure_model.tex <==
\begin{figure*}[tb]
    \centering
    \tikzset{
        ncbar angle/.initial=90,
        ncbar/.style={
            to path=(\tikztostart)
            -- ($(\tikztostart)!#1!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztotarget)$)
            -- ($(\tikztotarget)!($(\tikztostart)!#1!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztotarget)$)!\pgfkeysvalueof{/tikz/ncbar angle}:(\tikztostart)$)
            -- (\tikztotarget)
        },
        ncbar/.default=0.5cm,
    }
    
    \tikzset{round left paren/.style={ncbar=0.5cm,out=100,in=-100}}
    \tikzset{round right paren/.style={ncbar=0.5cm,out=80,in=-80}}
    
    \centering
    \scalebox{0.85}{
    \begin{tikzpicture}[scale=0.5]
        % underlay tau
        \draw[fill=cyan!15,draw=cyan!35,rounded corners] (-2.5,-2.25) rectangle ++ (19,-7.5);
        %% nodes
        % images
        \draw[fill=orange!15,draw=orange!35,rounded corners] (-8,3.25) rectangle ++ (4,-5);
        \node[anchor=center] (x0) at (-6,0) {\includegraphics[width=1.5cm]{plots/figure1/x_T.png}};
        \draw[fill=orange!15,draw=orange!35,rounded corners] (0.5,3.25) rectangle ++ (4,-5);
        \node[anchor=south] (x0label) at (x0.north) {$\mathbf{x}^{(\alpha)}_T$};
        \node[anchor=center] (x1) at (2.5,0) {\includegraphics[width=1.5cm]{plots/figure1/x_i.png}};
        \node[anchor=south] (x1label) at (x1.north) {$\mathbf{x}^{(\alpha)}_{T-1}$};
        \node[anchor=center] (xi) at (11.25,0) {$\cdots$};
        % text
        \draw[fill=orange!15,draw=orange!35,rounded corners] (16,3.25) rectangle ++ (4,-5);
        \node[anchor=center] (xT) at (18,0) {\includegraphics[width=1.5cm]{plots/figure1/x_0.png}};
        \node[anchor=south] (xTlabel) at (xT.north) {$\mathbf{x}^{(\alpha)}_0$};
        % conditioning
        \node[anchor=west] (clabel) at (2, -3.5) {};%conditioning};
        % wind prior
        \node[anchor=east] (c1) at (4.8, -4) {\includegraphics[width=1cm]{plots/figure1/feature_9.png}};
        \node[anchor=west, text width=7cm] (c1label) at (5, -4) {low resolution ECMWF mean $\x$};
        % weather prior
        \node[anchor=east, opacity=.5] (c2) at (2.8, -6.2) {\includegraphics[width=1cm]{plots/figure1/static_0.png}};
        \node[anchor=east, opacity=.5] (c2) at (3, -6.3) {\includegraphics[width=1cm]{plots/figure1/static_1.png}};
        \node[anchor=east, opacity=.5] (c2) at (3.2, -6.4) {\includegraphics[width=1cm]{plots/figure1/feature_0.png}};
        \node[anchor=east, opacity=.5] (c2) at (3.4, -6.5) {\includegraphics[width=1cm]{plots/figure1/feature_1.png}};
        \node[anchor=east, opacity=.5] (c2) at (3.6, -6.6) {\includegraphics[width=1cm]{plots/figure1/feature_2.png}};
        \node[anchor=east, opacity=.5] (c2) at (3.8, -6.7) {\includegraphics[width=1cm]{plots/figure1/feature_3.png}};
        \node[anchor=east, opacity=.5] (c2) at (4, -6.8) {\includegraphics[width=1cm]{plots/figure1/feature_4.png}};
        \node[anchor=east, opacity=.5] (c2) at (4.2, -6.9) {\includegraphics[width=1cm]{plots/figure1/feature_5.png}};
        \node[anchor=east, opacity=.5] (c2) at (4.4, -7) {\includegraphics[width=1cm]{plots/figure1/feature_6.png}};
        \node[anchor=east, opacity=.5] (c2) at (4.6, -7.1) {\includegraphics[width=1cm]{plots/figure1/feature_7.png}};
        \node[anchor=east, opacity=1.0] (c2) at (4.8, -7.2) {\includegraphics[width=1cm]{plots/figure1/feature_8.png}};
        \node[anchor=west, text width=6cm] (c2label) at (5, -6.8) {weather \& regional priors $R$};
        % scaling factor
        \node[anchor=east] (c3) at (4.8, -9) {\textcolor{black}{$\{\alpha, l\}$}};
        \node[anchor=west] (c3label) at (5, -9) {scaling factor \& lead time};
        \node[anchor=center] (emb) at (-1.75, -6) {$\tau = $};
        %% dummy nodes for drawing
        % conditioning
        \node[inner sep=0] (p1) at (-2.75, -9){};
        \node[inner sep=0] (p2) at (-2.75, -2){};
        \node[inner sep=0] (p3) at (18, -2){};
        % inputs
        \node[inner sep=0] (px0) at (3, -2){};
        \node[inner sep=0] (px1) at (9, -2){};
        \node[inner sep=0] (pxi) at (14, -2){};
        % \node[inner sep=0] (pxT) at (20, -2){};
        %% braces 
        \draw[thick, decorate, decoration={calligraphic brace,amplitude=15}](0,-9.5) -- (0,-2.5);
        \draw[thick, decorate, decoration={calligraphic brace,amplitude=15}](15,-2.5) -- (15,-9.5);
        % drawing paths
        \draw[-latex, thick] (x0) -- (x1);
        \draw[-latex, thick] (x1) -- (xi);
        \draw[-latex, thick] (xi) -- (xT);
        % score function
        % underlay solver
        \draw[fill=gray!15, draw=gray!35, rounded corners] (-3.5,1.25) rectangle ++ (3.5,-1.75);
        \draw[fill=gray!15, draw=gray!35, rounded corners] (4.75,1.25) rectangle ++ (5,-1.75);
        \draw[fill=gray!15, draw=gray!35, rounded corners] (12.25,1.25) rectangle ++ (3.45,-1.75);
        % step T
        \node[anchor=center] (sT) at (-1.75,-0){\tiny$\scoreF(\textcolor{orange}{\x^{(\alpha)}_T}, t_T, \textcolor{cyan!100}{\tau})$};
        \node[anchor=center] at ($(sT) + (0,0.75)$) {\tiny solver step for};
        % step T-1
        \node[anchor=center] (sT-1) at (7.25,-0){\tiny$\scoreF(\textcolor{orange}{\x^{(\alpha)}_{T-1}}, t_{T-1}, \textcolor{cyan!100}{\tau})$};
        \node[anchor=center] at ($(sT-1) + (0,0.75)$) {\tiny solver step for };
        % step 1
        \node[anchor=center, rounded corners] (s1) at (14,-0){\tiny$\scoreF(\textcolor{orange}{\x^{(\alpha)}_1}, t_1, \textcolor{cyan!100}{\tau})$};
        \node[anchor=center] at ($(s1) + (0,0.75)$) {\tiny solver step for };
        % paths
        \draw[-, thick] (emb) -- ($(emb) + (0,4)$) -| ($(sT)-(0,0.5)$);
        \draw[-, thick] (emb) -- ($(emb) + (0,4)$) -| ($(sT-1)-(0,0.5)$);
        \draw[-, thick] (emb) -- ($(emb) + (0,4)$) -| ($(s1)-(0,0.5)$);
    \end{tikzpicture}
    }
        \caption{The \textit{DiffScale} Diffusion model with classifier free guidance $\tau$. Arrows symbolize numerical solver steps for the respective score, solving the reverse process to generate $\x^{(\alpha)}$ given $\x$.}
    \label{fig:model}
\end{figure*}
